Noise Optimization for MKIDs with Different Design Geometries and Material Selections

The separation and optimization of noise components is critical to microwave-kinetic inductance detector (MKID) development. We analyze the effect of several changes to the lumped-element inductor and interdigitated capacitor geometry on the noise performance of a series of MKIDs intended for millimeter-wavelength experiments. We extract the contributions from two-level system noise in the dielectric layer, the generation-recombination noise intrinsic to the superconducting thin-film, and system white noise from each detector noise power spectrum and characterize how these noise components depend on detector geometry, material, and measurement conditions such as driving power and temperature. We observe a reduction in the amplitude of two-level system noise with both an elevated sample temperature and an increased gap between the fingers within the interdigitated capacitors for both aluminum and niobium detectors. We also verify the expected reduction of the generation-recombination noise and associated quasiparticle lifetime with reduced inductor volume. This study also iterates over different materials, including aluminum, niobium, and aluminum manganese, and compares the results with an underlying physical model.

==> Noise Optimization for MKIDs with Different Design Geometries and Material Selections/authors.tex <==
\author{
Z.~Pan\textsuperscript{1},
K.~R.~Dibert\textsuperscript{2, 3},
J.~Zhang\textsuperscript{1},
P.~S.~Barry\textsuperscript{4,1},
A.~J.~Anderson\textsuperscript{2, 3, 5},
A.~N.~Bender\textsuperscript{1},
B.~A.~Benson\textsuperscript{2, 3, 5},
T.~Cecil\textsuperscript{1},
C.~L.~Chang\textsuperscript{1, 2, 3},
R.~Gualtieri\textsuperscript{1},
J.~Li\textsuperscript{1},
M.~Lisovenko\textsuperscript{1},
V.~Novosad\textsuperscript{1}, 
M.~Rouble\textsuperscript{6},
G.~Wang\textsuperscript{1},
and~V.~Yefremenko\textsuperscript{1},
% Affiliations

\institute{
\textsuperscript{1}{Argonne National Laboratory, 9700 South Cass Avenue., Argonne, IL, 60439, USA} \\
\textsuperscript{2}{Dept. of Astronomy \& Astrophysics, U. Chicago, 5640 South Ellis Avenue, Chicago, IL, 60637, USA} \\
\textsuperscript{3}{Kavli Institute for Cosmological Physics, U. Chicago, 5640 South Ellis Avenue, Chicago, IL, 60637, USA} \\
\textsuperscript{4}{School of Physics and Astronomy, Cardiff University, Cardiff CF24 3YB, UK} \\
\textsuperscript{5}{Fermi National Accelerator Laboratory, MS209, P.O. Box 500, Batavia, IL, 60510, USA} \\
\textsuperscript{6}{Department of Physics, McGill University, 3600 Rue University, Montreal, Quebec H3A 2T8, Canada} \\
}

}


==> authors.tex <==
\author{
Z.~Pan\textsuperscript{1},
K.~R.~Dibert\textsuperscript{2, 3},
J.~Zhang\textsuperscript{1},
P.~S.~Barry\textsuperscript{4,1},
A.~J.~Anderson\textsuperscript{2, 3, 5},
A.~N.~Bender\textsuperscript{1},
B.~A.~Benson\textsuperscript{2, 3, 5},
T.~Cecil\textsuperscript{1},
C.~L.~Chang\textsuperscript{1, 2, 3},
R.~Gualtieri\textsuperscript{1},
J.~Li\textsuperscript{1},
M.~Lisovenko\textsuperscript{1},
V.~Novosad\textsuperscript{1}, 
M.~Rouble\textsuperscript{6},
G.~Wang\textsuperscript{1},
and~V.~Yefremenko\textsuperscript{1},
% Affiliations

\institute{
\textsuperscript{1}{Argonne National Laboratory, 9700 South Cass Avenue., Argonne, IL, 60439, USA} \\
\textsuperscript{2}{Dept. of Astronomy \& Astrophysics, U. Chicago, 5640 South Ellis Avenue, Chicago, IL, 60637, USA} \\
\textsuperscript{3}{Kavli Institute for Cosmological Physics, U. Chicago, 5640 South Ellis Avenue, Chicago, IL, 60637, USA} \\
\textsuperscript{4}{School of Physics and Astronomy, Cardiff University, Cardiff CF24 3YB, UK} \\
\textsuperscript{5}{Fermi National Accelerator Laboratory, MS209, P.O. Box 500, Batavia, IL, 60510, USA} \\
\textsuperscript{6}{Department of Physics, McGill University, 3600 Rue University, Montreal, Quebec H3A 2T8, Canada} \\
}

}

